HAM: Hybrid Associations Models for Sequential Recommendation

Sequential recommendation aims to identify and recommend the next few items for a user that the user is most likely to purchase/review, given the user's purchase/rating trajectories. It becomes an effective tool to help users select favorite items from a variety of options. In this manuscript, we developed hybrid associations models (HAM) to generate sequential recommendations using three factors: 1) users' long-term preferences, 2) sequential, high-order and low-order association patterns in the users' most recent purchases/ratings, and 3) synergies among those items. HAM uses simplistic pooling to represent a set of items in the associations, and element-wise product to represent item synergies of arbitrary orders. We compared HAM models with the most recent, state-of-the-art methods on six public benchmark datasets in three different experimental settings. Our experimental results demonstrate that HAM models significantly outperform the state of the art in all the experimental settings, with an improvement as much as 46.6%. In addition, our run-time performance comparison in testing demonstrates that HAM models are much more efficient than the state-of-the-art methods, and are able to achieve significant speedup as much as 139.7 folds.

==> tables/ablation_Books.tex <==
\begin{table}[!h]
\footnotesize
  \caption{\mbox{Ablation Study of \methodCorm on Books in \CUT}}
    \label{tbl:ablaBooks}
  \centering
  %\vspace{-5pt}
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{8pt}}c@{\hspace{4pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
        @{\hspace{4pt}}r@{\hspace{8pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
        @{\hspace{10pt}}r@{\hspace{8pt}}
        @{\hspace{4pt}}r@{\hspace{4pt}}
    @{\hspace{4pt}}r@{\hspace{8pt}}
        }
        \toprule
        w/o & $d$ & $\LL$ & $\M$ & $\T$ & $p$ & Recall@5 & Recall@10 \\
        \midrule
        %\multirow{6}{*}{R@10}
        none & 400 & 9 & 2 & 7 & 2 & \textbf{$\mathclap{^{\dagger~}}$0.0412} 
        & \textbf{$\mathclap{^{\dagger~}}$0.0630}\\
        \midrule
        $\sse$ & 400 & 3 & 0 & 8 & 2 & 0.0367 & 0.0579\\
        \midrule
        $\user$ & 400 & 7 & 1 & 5 & 2 & 0.0373 & 0.0548\\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}[normal,flushleft]
      \begin{scriptsize}
      \item
          In this table, $d$, $\LL$/$\M$, $\T$ and $p$ are 
	  the dimension of embeddings, number of items in high-order/low-order associations,
          number of items to calculate recommendation errors during training
          and the order of item synergies.
	  The best performance overall is \textbf{$\mathclap{^{\dagger~}}$bold}; 
          the best performance in each row block is \textbf{bold}; and 
          The ``w/o'' column presents the factor ablated:
          the row corresponding to ``none" represents the full model without any ablation; 
          the row block corresponding to $\sse$ represents the results when the low-order association is ablated (i.e., \xia{$\M=0$});  
 	  the row block corresponding to $\user$ represents the results when the users' general preferences is ablated. 
	  %          $\user$ is the representation of the general preferences of users
	  %\xia{please use the format of this table to format others...}
          \par
      \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
  %\vspace{-8pt}
\end{table}


==> tables/ablation_Child.tex <==
\begin{table}[!h]
\footnotesize
  \caption{\mbox{Ablation Study of \methodCorm on Children in \CUT}}
    \label{tbl:ablaChild}
  \centering
  %\vspace{-5pt}
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{8pt}}c@{\hspace{4pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
        @{\hspace{4pt}}r@{\hspace{8pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
        @{\hspace{10pt}}r@{\hspace{8pt}}
        @{\hspace{4pt}}r@{\hspace{4pt}}
    @{\hspace{4pt}}r@{\hspace{8pt}}
        }
        \toprule
        w/o & $d$ & $\LL$ & $\M$ & $\T$ & $p$ & Recall@5 & Recall@10 \\
        \midrule
        %\multirow{6}{*}{R@10}
        none & 400 & 6 & 1 & 4 & 3 & \textbf{$\mathclap{^{\dagger~}}$0.0921} 
        & \textbf{$\mathclap{^{\dagger~}}$0.1393}\\
        \midrule
        $\sse$ & 600 & 3 & 0 & 4 & 3 & 0.0854 & 0.1324\\
        \midrule
        $\user$ & 200 & 6 & 1 & 4 & 2 & 0.0910 & 0.1386\\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}[normal,flushleft]
      \begin{scriptsize}
      \item
          In this table, $d$, $\LL$/$\M$, $\T$ and $p$ are 
	  the dimension of embeddings, number of items in high-order/low-order associations,
          number of items to calculate recommendation errors during training
          and the order of item synergies.
	  The best performance overall is \textbf{$\mathclap{^{\dagger~}}$bold}; 
          the best performance in each row block is \textbf{bold}; and 
          The ``w/o'' column presents the factor ablated:
          the row corresponding to ``none" represents the full model without any ablation; 
          the row block corresponding to $\sse$ represents the results when the low-order association is ablated (i.e., \xia{$\M=0$});  
 	  the row block corresponding to $\user$ represents the results when the users' general preferences is ablated. 
	  %          $\user$ is the representation of the general preferences of users
	  %\xia{please use the format of this table to format others...}
          \par
      \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
  %\vspace{-8pt}
\end{table}


==> tables/ablation_Comics.tex <==
\begin{table}[!h]
\footnotesize
  \caption{\mbox{Ablation Study of \methodCorm on Comics in \CUT}}
    \label{tbl:ablaComics}
  \centering
  %\vspace{-5pt}
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{0pt}}c@{\hspace{8pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
    @{\hspace{8pt}}r@{\hspace{0pt}}
        }
        \toprule
        w/o & $d$ & $\LL$ & $\M$ & $\T$ & $p$ & Recall@5 & Recall@10 \\
        \midrule
        none & 400 & 7 & 2 & 5 & 3 & 0.1385 & 0.1945\\
        \midrule
        \multirow{5}{*}{{{\centering $\sse$}}}
        & 400 & 4 & 0 & 3 & 3 & \textbf{0.1233} & \textbf{0.1751}\\
        & 400 & 5 & 0 & 3 & 3 & 0.1220 & 0.1741\\
        & \underline{400} & \underline{6} & \underline{0} & \underline{3} & \underline{3}
        & \underline{0.1205} & \underline{0.1726}\\
        & 400 & 7 & 0 & 3 & 3 & 0.1195 & 0.1710\\
        & 400 & 8 & 0 & 3 & 3 & 0.1169 & 0.1687\\
        \midrule
        \multirow{5}{*}{{{\centering $\user$}}}
        & 200 & 5 & 1 & 6 & 2 & \textbf{$\mathclap{^{\dagger~}}$0.1438} & 0.1976\\
        & 200 & 6 & 1 & 6 & 2 & 0.1436 & 0.1974\\
        & \underline{200} & \underline{7} & \underline{1} & \underline{6} & \underline{2}
        & \underline{0.1422} & \underline{0.1974}\\
        & 200 & 8 & 1 & 6 & 2 & \textbf{$\mathclap{^{\dagger~}}$0.1438} & \textbf{$\mathclap{^{\dagger~}}$0.1983}\\
        & 200 & 9 & 1 & 6 & 2 & 0.1430 & 0.1979\\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}[normal,flushleft]
      \begin{scriptsize}
      \item
          In this table, $d$, $\LL$/$\M$, $\T$ and $p$ are 
	  the dimension of embeddings, number of items in high-order/low-order associations,
          number of items to calculate recommendation errors during training
          and the order of item synergies.
	  The best performance overall is \textbf{$\mathclap{^{\dagger~}}$bold}
          and the best performance in each row block is \textbf{bold}.
          The selected best parameters and corresponding results are \underline{underlined}.
          The ``w/o'' column presents the component to be removed in each row block.
          $\sse$ is the representation of the low-order associations.
          $\user$ is the representation of the general preferences of users
          \par
      \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
  %\vspace{-8pt}
\end{table}


==> tables/ablation_ML1M.tex <==
\begin{table}[!h]
\footnotesize
  \caption{\mbox{Ablation Study of \methodCorm on ML-1M in \CUT}}
    \label{tbl:ablaML1M}
  \centering
  %\vspace{-5pt}
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{8pt}}c@{\hspace{4pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
        @{\hspace{4pt}}r@{\hspace{8pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
        @{\hspace{10pt}}r@{\hspace{8pt}}
        @{\hspace{4pt}}r@{\hspace{4pt}}
    @{\hspace{4pt}}r@{\hspace{8pt}}
        }
        \toprule
        w/o & $d$ & $\LL$ & $\M$ & $\T$ & $p$ & Recall@5 & Recall@10 \\
        \midrule
        %\multirow{6}{*}{R@10}
        none & 400 & 7 & 2 & 3 & 3 & \textbf{$\mathclap{^{\dagger~}}$0.0793} 
        & \textbf{$\mathclap{^{\dagger~}}$0.1330}\\
        \midrule
        $\sse$ & 600 & 5 & 0 & 1 & 3 & 0.0763 & 0.1291\\
        \midrule
        $\user$ & 200 & 9 & 2 & 3 & 2 & 0.0792 & 0.1322\\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}[normal,flushleft]
      \begin{scriptsize}
      \item
          In this table, $d$, $\LL$/$\M$, $\T$ and $p$ are 
	  the dimension of embeddings, number of items in high-order/low-order associations,
          number of items to calculate recommendation errors during training
          and the order of item synergies.
	  The best performance overall is \textbf{$\mathclap{^{\dagger~}}$bold}; 
          the best performance in each row block is \textbf{bold}; and 
          The ``w/o'' column presents the factor ablated:
          the row corresponding to ``none" represents the full model without any ablation; 
          the row block corresponding to $\sse$ represents the results when the low-order association is ablated (i.e., \xia{$\M=0$});  
 	  the row block corresponding to $\user$ represents the results when the users' general preferences is ablated. 
	  %          $\user$ is the representation of the general preferences of users
	  %\xia{please use the format of this table to format others...}
          \par
      \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
  %\vspace{-8pt}
\end{table}


==> tables/distribution_combine.tex <==
\begin{table*}
%\begin{minipage}[!t]{0.33\linewidth}
%  \vspace{-18pt}
%  \centering
%  \input{./plots/data_distribution/data_distribution.tex}
%  \vspace{-10pt}
%  \captionof{figure}{Item Frequency Distribution}
%  \label{fig:total_distribution}
%  \vspace{-10pt}
%\end{minipage}
%
\begin{minipage}{0.49\linewidth}
%  \captionsetup{format=myformat}
  \centering
\captionof{table}{\methodMean Parameter Study  \newline (\CUS, $\M$=$2$, $\T$=$3$)}
  \label{tbl:parameterT}
  %\centering
  %\vspace{-6pt}
  \begin{threeparttable}

     \begin{footnotesize}
        \begin{tabular}{
        @{\hspace{0pt}}c@{\hspace{2pt}}
        %
        @{\hspace{2pt}}c@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        %
        @{\hspace{0pt}}r@{\hspace{0pt}}
        %
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{0pt}}
        }
        \toprule
        \multirow{2}{*}{$\LL$}
        &\multicolumn{2}{c}{CDs} && \multicolumn{2}{c}{Comics}\\
        \cline{2-3}\cline{5-6}
        & \scriptsize{Recall@5} & \scriptsize{Recall@10} && \scriptsize{Recall@5} & \scriptsize{Recall@10}\\
        \midrule
         3 & 0.0358 & 0.0556 && 0.2384 & 0.3022\\
         4 & \textbf{0.0369} & \textbf{0.0583} && 0.2402 & 0.3043\\
         5 & 0.0366 & 0.0567 && \textbf{0.2414} & \textbf{0.3065}\\
         6 & 0.0360 & 0.0572 && 0.2392 & 0.3063\\
        \bottomrule
      \end{tabular}
   \end{footnotesize}
      %\begin{tablenotes}[normal,flushleft]
      %\begin{scriptsize}
      %\item
      %    The best performance for each $|T|$ is \underline{underlined}.
      %    The best performance across all $|T|$ values is \textbf{bold}.
      %    \par
      %\end{scriptsize}
      %\end{tablenotes}
  \end{threeparttable}
\end{minipage}
%
\begin{minipage}{0.49\linewidth}
%\captionsetup{format=myformat}
\caption{\methodMean Parameter Study \newline (\LOS, $\M$=$2$, $\T$=$3$)}
  \label{tbl:parameterO}
  \centering       
  %\vspace{-5pt}   
  \begin{threeparttable}
   \begin{footnotesize}
      \begin{tabular}{
        @{\hspace{0pt}}c@{\hspace{2pt}}
        %
        @{\hspace{2pt}}c@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        %
        @{\hspace{0pt}}r@{\hspace{0pt}}
        %
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{0pt}}
        }
        \toprule
        \multirow{2}{*}{$\LL$}
        &\multicolumn{2}{c}{CDs} && \multicolumn{2}{c}{Comics}\\
        \cline{2-3}\cline{5-6}
        & \scriptsize{Recall@5} & \scriptsize{Recall@10} && \scriptsize{Recall@5} & \scriptsize{Recall@10}\\
        \midrule
%         3 & 0.0345 & 0.0541 && 0.1791 & 0.2289\\
         4 & 0.0343 & 0.0544 && 0.1818 & 0.2317\\
         5 & \textbf{0.0357} & \textbf{0.0565} && \textbf{0.1823} & \textbf{0.2331}\\
         6 & 0.0355 & 0.0550 && 0.1821 & 0.2314\\
        \bottomrule
      \end{tabular}
   \end{footnotesize}
  \end{threeparttable}
\end{minipage}
%\vspace{-6pt}
\end{table*}


==> tables/notations.tex <==
\begin{table}[!t]
  \caption{Notations}
  \label{tbl:notations}
  \centering
  \begin{threeparttable}
    \begin{footnotesize}
      \begin{tabular}{
	@{\hspace{0pt}}l@{\hspace{30pt}}
	@{\hspace{30pt}}l@{\hspace{0pt}}          
	}
        \toprule
        notations & meanings \\
        \midrule
        $m$/$n$ &  number of users/items\\
        $\sequences_i$ & purchase/rating sequence of user $i$ \\
	$\sequences_i(t, l)$ & a length-$l$ subsequence of $\sequences_i$ starting\\
	& from the $t$-th purchase/rating\\
        \U &  user embedding matrix \\
        \EM &  item embedding matrix \\
        \QM &  candidate item embedding matrix \\
%        $k$ & the dimension of the embeddings \\
        $\rs_{ij}$ & the recommendation score of user $i$ \\
                   &  on item $j$ \\
        $n_h$/$n_l$ & the number of items of high-order/\\
                   & low-order sequential association \\
        {$n_p$}  & the number of next items to be \\ 
                 & recommended  during training \\
       \bottomrule
      \end{tabular}
  \end{footnotesize}
  \end{threeparttable}
\end{table}


==> tables/parameter.tex <==
\begin{table}[!h]
  \caption{Parameter Study in \CUT ($|M| = 2$)}
  \label{tbl:parameter}
  \centering
  \vspace{-5pt}
  \begin{threeparttable}
      \begin{tabular}{
	@{\hspace{0pt}}c@{\hspace{2pt}}
	@{\hspace{2pt}}c@{\hspace{2pt}}          
	%
        @{\hspace{4pt}}r@{\hspace{4pt}}
        @{\hspace{4pt}}r@{\hspace{8pt}}
        %
        @{\hspace{0pt}}r@{\hspace{0pt}}
        %
	@{\hspace{8pt}}r@{\hspace{4pt}}
    	@{\hspace{4pt}}r@{\hspace{2pt}}
	}
        \toprule
        \multirow{2}{*}{$|L|$} & \multirow{2}{*}{$|T|$} 
        &\multicolumn{2}{c}{CDs} && \multicolumn{2}{c}{Comics}\\
        \cline{3-4}\cline{6-7}
        && \scriptsize{Recall@5} & \scriptsize{Recall@10} && \scriptsize{Recall@5} & \scriptsize{Recall@10}\\
        \midrule
        \multirow{3}{*}{3}
        & 1 & 0.0318 & 0.0499 && 0.1156 & 0.1649\\
        & 2 & 0.0324 & 0.0501 && 0.1237 & 0.1750\\
        & 3 & 0.0324 & 0.0504 && 0.1253 & 0.1774\\
        \midrule
                \multirow{3}{*}{4}
         & 1  & 0.0317 & \underline{0.0507} && 0.1165 & 0.1676\\
         & 2  & \textbf{0.0332} & \underline{0.0507} && 0.1244 & 0.1763\\
         & 3  & 0.0324 & 0.0505 && \underline{0.1270} & \underline{0.1795}\\
        \midrule
        \multirow{3}{*}{5}
         & 1  & 0.0323 & 0.0505 && 0.1166 & 0.1677\\
         & 2  & 0.0323 & \underline{0.0507} && 0.1259 & 0.1786\\
         & 3  & \underline{0.0327} & \textbf{0.0508} && \textbf{0.1284} & \textbf{0.1814}\\
        \bottomrule
      \end{tabular}
            \begin{tablenotes}[normal,flushleft]
      \begin{scriptsize}
      \item 
          The best performance for each $|L|$ is \underline{underlined}.
          The best performance across all $|L|$ values is \textbf{bold}. 
          \xia{Bo: in this table, need results for $|L|=6$, and $|L|=5$ and $|T| = 4$}
          \par
      \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
\end{table}


==> tables/parameter_Caser.tex <==
\begin{table}[!h]
\footnotesize
  \caption{\mbox{Best Parameters for \Caser}}
  \centering
  \label{tbl:para:caser}
  %\vspace{-10pt}
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{10pt}}l@{\hspace{10pt}}
        @{\hspace{10pt}}l@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        }
        \toprule
        Setting & Dataset & $d$ & $L$ & $T$ & $nv$ & $nh$\\
        \midrule
        %\multirow{6}{*}{R@10}
%        \multirow{6}{*}{{{\centering \CUT/\CUS}}}
\multirow{6}{*}{\parbox{0.1\linewidth}{\CUT  \CUS}}
        & CDs      & 200 & 5 & 4 & 2 & 16\\
	& Books    & 200 & 6 & 4 & 2 & 8\\
        & Children & 100 & 4 & 4 & 2 & 16\\
        & Comics   & 100 & 4 & 4 & 2 & 16\\
        & ML-20M   & 100 & 6 & 2 & 4 & 8\\
        & ML-1M    & 200 & 6 & 2 & 2 & 8\\
        \midrule
        %\multirow{6}{*}{N@10}
        \multirow{6}{*}{{{\centering \LOS}}}
        & CDs      & 200 & 4 & 4 & 2 & 16\\
        & Books    & 200 & 5 & 3 & 2 & 8\\
        & Children & 200 & 4 & 4 & 2 & 8\\
        & Comics   & 200 & 4 & 4 & 2 & 8\\
        & ML-20M   & 200 & 4 & 4 & 2 & 8\\
        & ML-1M    & 200 & 5 & 2 & 2 & 16\\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}[normal,flushleft]
      \begin{scriptsize}
      \item
          In this table, $d$, $T$, $L$, $nv$ and $nh$ are
          the dimension of embeddings, 
          the length of the subsequences,
          the number of items used as targets in training, 
          the number of vertical filters and the number of horizontal filters.
          \par
      \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
\end{table}


==> tables/parameter_HAM.tex <==
\begin{table}[!h]
\footnotesize
  \caption{\mbox{Best Parameters for \methodCorm}}
  \centering
  \label{tbl:para:ham}
  %\vspace{-10pt}
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{10pt}}p{0.1\linewidth}@{\hspace{10pt}}
        @{\hspace{10pt}}l@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        }
        \toprule
        Setting & Dataset & $d$ & $\LL$ & $\M$ & $\T$ & $p$ \\
        \midrule
        %\multirow{6}{*}{R@10}
        \multirow{6}{*}{\parbox{0.1\linewidth}{\CUT  \CUS}}
        %\multirow{6}{*}{{{\centering \CUT/\CUS}}}
        & CDs      & 400 & 5 & 2 & 3 & 2\\
	& Books    & 400 & 9 & 2 & 7 & 2\\
        & Children & 400 & 6 & 1 & 4 & 3\\
        & Comics   & 400 & 7 & 2 & 5 & 3\\
        & ML-20M   & 400 & 9 & 3 & 2 & 3\\
        & ML-1M    & 400 & 7 & 2 & 3 & 3\\
        \midrule
        %\multirow{6}{*}{N@10}
        \multirow{6}{*}{{{\centering \LOS}}}
        & CDs      & 400 & 4 & 2 & 7 & 2\\
        & Books    & 400 & 9 & 2 & 9 & 2\\
        & Children & 400 & 6 & 1 & 4 & 3\\
        & Comics   & 400 & 7 & 1 & 5 & 3\\
        & ML-20M   & 400 & 8 & 3 & 3 & 3\\
        & ML-1M    & 400 & 8 & 2 & 2 & 3\\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}[normal,flushleft]
      \begin{scriptsize}
      \item
          In this table, $d$, $\LL$/$\M$, $\T$ and $p$ are
          the dimension of embeddings, number of items in high-order/low-order associations,
          number of items to calculate recommendation errors during training
          and the order of item synergies.
          \par
      \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
\end{table}


==> tables/parameter_HGN.tex <==
\begin{table}[!h]
\footnotesize
  \caption{\mbox{Best Parameters for \HGN}}
  \centering
  \label{tbl:para:hgn}
  %\vspace{-16pt}
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{16pt}}l@{\hspace{16pt}}
        @{\hspace{16pt}}l@{\hspace{16pt}}
        @{\hspace{16pt}}r@{\hspace{16pt}}
        @{\hspace{16pt}}r@{\hspace{16pt}}
        @{\hspace{16pt}}r@{\hspace{16pt}}
        }
        \toprule
        Setting & Dataset & $d$ & $L$ & $T$\\
        \midrule
        %\multirow{6}{*}{R@10}
%        \multirow{6}{*}{{{\centering \CUT/\CUS}}}
\multirow{6}{*}{\parbox{0.1\linewidth}{\CUT  \CUS}}
        & CDs      & 200 & 5 & 2\\
	& Books    & 400 & 4 & 4\\
        & Children & 200 & 2 & 4\\
        & Comics   & 200 & 2 & 6\\
        & ML-20M   & 100 & 5 & 3\\
        & ML-1M    & 100 & 4 & 4\\
        \midrule
        %\multirow{6}{*}{N@10}
        \multirow{6}{*}{{{\centering \LOS}}}
        & CDs      & 200 & 4 & 3\\
        & Books    & 400 & 2 & 6\\
        & Children & 100 & 2 & 5\\
        & Comics   & 200 & 2 & 5\\
        & ML-20M   & 100 & 6 & 3\\
        & ML-1M    & 100 & 3 & 4\\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}[normal,flushleft]
      \begin{scriptsize}
      \item
          In this table, $d$, $L$ and $T$ are
          the dimension of embeddings, 
          the length of the subsequences
          and the number of items used as targets in training.
          \par
      \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
\end{table}


==> tables/parameter_SASRec.tex <==
\begin{table}[!h]
\footnotesize
  \caption{\mbox{Best Parameters for \SASRec}}
  \centering
  \label{tbl:para:sasrec}
  %\vspace{-16pt}
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{16pt}}l@{\hspace{16pt}}
        @{\hspace{16pt}}l@{\hspace{16pt}}
        @{\hspace{16pt}}r@{\hspace{16pt}}
        @{\hspace{16pt}}r@{\hspace{16pt}}
        @{\hspace{16pt}}r@{\hspace{16pt}}
        }
        \toprule
        Setting & Dataset & $d$ & $n$ & $h$\\
        \midrule
        %\multirow{6}{*}{R@10}
%        \multirow{6}{*}{{{\centering \CUT/\CUS}}}
\multirow{6}{*}{\parbox{0.1\linewidth}{\CUT  \CUS}}
        & CDs      & 400 & 600 & 1\\
	& Books    & 400 & 600 & 1\\
        & Children & 400 & 200 & 1\\
        & Comics   & 400 & 400 & 1\\
        & ML-20M   & 400 & 400 & 4\\
        & ML-1M    & 200 & 600 & 1\\
        \midrule
        %\multirow{6}{*}{N@10}
        \multirow{6}{*}{{{\centering \LOS}}}
        & CDs      & 400 & 400 & 4\\
        & Books    & 400 & 400 & 1\\
        & Children & 400 & 200 & 1\\
        & Comics   & 600 & 600 & 1\\
        & ML-20M   & 400 & 400 & 4\\
        & ML-1M    & 200 & 600 & 2\\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}[normal,flushleft]
      \begin{scriptsize}
      \item
          In this table, $d$, $n$ and $h$ are
          the dimension of embeddings, the maximum sequence length and
          the number of head of the multi-head attention.
          \\
          \par
      \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
\end{table}


==> tables/parameter_T.tex <==
\begin{table}[!h]
  \caption{Parameter Study}
  \label{tbl:parameterT}
  \centering
  \vspace{-5pt}
  \begin{threeparttable}
      \begin{tabular}{
	@{\hspace{0pt}}c@{\hspace{2pt}}
	@{\hspace{2pt}}c@{\hspace{2pt}}
        @{\hspace{2pt}}c@{\hspace{2pt}}
	%
        @{\hspace{4pt}}c@{\hspace{4pt}}
        @{\hspace{4pt}}r@{\hspace{8pt}}
        %
        @{\hspace{0pt}}r@{\hspace{0pt}}
        %
	@{\hspace{8pt}}r@{\hspace{4pt}}
        @{\hspace{4pt}}r@{\hspace{2pt}}
	}
        \toprule
        \multirow{2}{*}{experiment} & \multirow{2}{*}{$|L|$} & \multirow{2}{*}{$|T|$} 
        &\multicolumn{2}{c}{CDs} && \multicolumn{2}{c}{Comics}\\
        \cline{4-5}\cline{7-8}
        &&& \scriptsize{Recall@5} & \scriptsize{Recall@10} && \scriptsize{Recall@5} & \scriptsize{Recall@10}\\
        \midrule
        \multirow{3}{*}{CUS} & \multirow{3}{*}{3}
        & 3 & 0.0358 & 0.0556 && 0.2384 & 0.3022\\
        && 4 & \textbf{0.0369} & \textbf{0.0583} && 0.2402 & 0.3043\\
        && 5 & 0.0366 & 0.0567 && \textbf{0.2414} & \textbf{0.3065}\\
        \midrule
        \multirow{3}{*}{LOS} & \multirow{3}{*}{3}
        & 3 & 0.0345 & 0.0541 && 0.1791 & 0.2289\\ 
        && 4 & 0.0343 & 0.0544 && 0.1818 & 0.2317\\
        && 5 & \textbf{0.0357} & \textbf{0.0565} && \textbf{0.1823} & \textbf{0.2331}\\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}[normal,flushleft]
      \begin{scriptsize}
      \item
          The best performance for each $|L|$ is \underline{underlined}.
          The best performance across all $|L|$ values is \textbf{bold}.
          \par
      \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
\end{table}


==> tables/parameter_ablution.tex <==
\begin{table}[!h]
  \caption{Parameter Study Ablution ($|M| = 0$)}
  \label{tbl:ablution}
  \centering
  \vspace{-5pt}
  \begin{threeparttable}
    %\begin{large}
      \begin{tabular}{
	@{\hspace{0pt}}c@{\hspace{2pt}}
	@{\hspace{2pt}}c@{\hspace{2pt}}
        %  
	@{\hspace{4pt}}c@{\hspace{4pt}}
        @{\hspace{4pt}}r@{\hspace{8pt}}
        %
        @{\hspace{0pt}}r@{\hspace{0pt}}
        %
        @{\hspace{8pt}}r@{\hspace{4pt}}
	@{\hspace{4pt}}r@{\hspace{2pt}}
	}
        \toprule
        \multirow{2}{*}{$|L|$} & \multirow{2}{*}{$|T|$}
        &\multicolumn{2}{c}{CDs} & \multicolumn{2}{c}{Comics}\\
        \cline{3-4}\cline{6-7}
        && \scriptsize{Recall@5} & \scriptsize{Recall@10} && \scriptsize{Recall@5} & \scriptsize{Recall@10}\\
        \midrule
        \multirow{3}{*}{3}
        & 1 & 0.0300 & 0.0484 && 0.0993 & 0.1486 \\
        & 2 & \textbf{0.0302} & \textbf{0.0492} && 0.1075 & 0.1585 \\
        & 3 & \underline{0.0301} & 0.0481 && \textbf{0.1101} & \underline{0.1607} \\
        \midrule
        \multirow{3}{*}{4}
        & 1 & 0.0298 & 0.0483 && 0.0991 & 0.1481 \\
        & 2 & 0.0299 & \underline{0.0491} && 0.1071 & 0.1584 \\
        & 3 & 0.0296 & 0.0481 && \underline{0.1094} & \textbf{0.1608} \\
        \midrule
        \multirow{3}{*}{5}
        & 1 & 0.0286 & 0.0462 && 0.0982 & 0.1473 \\
        & 2 & 0.0291 & 0.0473 && 0.1067 & 0.1568 \\
        & 3 & 0.0293 & 0.0481 && 0.1081 & 0.1593 \\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}[normal,flushleft]
      \begin{scriptsize}
      \item
          The best performance for each $|L|$ is \underline{underlined}.
          The best performance across all $|L|$ values is \textbf{bold}.
          \par
      \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
\end{table}


==> tables/parameter_combine.tex <==
\begin{table}[t]
%\vspace{-3pt}
\begin{minipage}[t]{0.45\linewidth}
  %\captionsetup{format=myformat}
  \caption{Recall@$10$ for \methodMean Parameter Study (\CUT, $\M$=$2$)}
  \label{tbl:parameter}
  \centering
  %\vspace{-5pt}
  \begin{threeparttable}
    %\begin{footnotesize}
      \begin{tabular}{
        @{\hspace{0pt}}c@{\hspace{8pt}}
        @{\hspace{8pt}}c@{\hspace{8pt}}
        %
%        @{\hspace{1pt}}r@{\hspace{1pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
        %
        @{\hspace{8pt}}r@{\hspace{8pt}}
        %
%        @{\hspace{2pt}}r@{\hspace{1pt}}
        @{\hspace{8pt}}r@{\hspace{0pt}}
        }
        \toprule
        %\multirow{2}{*}{$\LL$} & \multirow{2}{*}{$\T$}
        %&\multicolumn{2}{c}{CDs} && \multicolumn{2}{c}{Comics}\\
        %\cline{3-4}\cline{6-7}
        %&& \scriptsize{Recall@5} 
        %&& \scriptsize{Recall@10} %&& \scriptsize{Recall@5} 
        %& \scriptsize{Recall@10}\\
        $\LL$ & $\T$ & CDs && Comics\\
        \midrule
%        \multirow{4}{*}{3}
%        & 1 & 0.0318 & 0.0499 && 0.1156 & 0.1649\\
%        & 2 & \underline{0.0324} & 0.0501 && 0.1237 & 0.1750\\
%        & 3 & \underline{0.0324} & 0.0504 && 0.1253 & 0.1774\\
%        & 4 & 0.0322 & \underline{0.0506} && \underline{0.1258} & \underline{0.1783}\\
%        & 5 & 0.0310 & 0.0499 && 0.1250 & 0.1781\\
%        \midrule
                \multirow{4}{*}{4}
%         & 1 & 0.0317 
         & 1 & \underline{0.0507}% && 0.1165 
         && 0.1676\\
         %& 2 & \underline{\textbf{0.0332}} 
         & 2 & \underline{0.0507}% && 0.1244 
         && 0.1763\\
         %& 3 & 0.0324 
         & 3 & 0.0505% && \underline{0.1270} 
         && \underline{0.1795}\\
         %& 4 & 0.0311 
         & 4 & 0.0499% && 0.1259 
         && 0.1792\\
  %       & 5 & 0.0316 & 0.0503 && 0.1257 & 0.1787\\
        \midrule
        \multirow{3}{*}{5}
         %& 1 & 0.0323 
         %& 1 & 0.0505% && 0.1166 
         %&& 0.1677\\
         %& 2 & 0.0323
         & 2 & {0.0507}% && 0.1259 
         && 0.1786\\
         %& 3 & \underline{0.0327} 
         & 3 & \underline{\textbf{0.0508}}% && \underline{\textbf{0.1284}} 
         && \underline{0.1814}\\
         %& 4 & 0.0311 
         & 4 & 0.0496 %&& 0.1279 
         && 0.1813\\
         %& 5 & 0.0308 & 0.0484 && 0.1262 & 0.1798\\
         \midrule
         \multirow{4}{*}{6}
         %& 1 & 0.0306 
         %& 1 & 0.0505% && 0.1174 
         %&& 0.1690\\
         %& 2 & \underline{0.0322} 
         & 2 & \underline{0.0507} %&& 0.1260 
         && 0.1787\\
         %& 3 & 0.0317 
         & 3 & 0.0498 %&& 0.1275 
         && 0.1813\\
         %& 4 & 0.0310 
         & 4 & 0.0487 %&& \underline{0.l283} 
         && \underline{\textbf{0.1823}}\\
         %& 5 & 0.0318 
         & 5 & 0.0498 %&& 0.1266 
         && 0.1807\\
        \bottomrule
      \end{tabular}
  %\end{footnotesize}
      \begin{tablenotes}[normal,flushleft]
      \begin{scriptsize}
      \item
          In these two tables, 
          the best performance for each $\LL$ is \underline{underlined}.
          The best performance across all $\LL$ values is \textbf{bold}.
          %\xia{Bo: in this table, need results for $|L|=6$, and $|L|=5$ and $|T| = 4$}
          \par
      \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
\end{minipage}
%
\hfill
%\quad
%
\begin{minipage}[t]{0.45\linewidth}
  %\captionsetup{format=myformat}
  \caption{Recall@$10$ for \methodMean Ablation Study (\CUT, $\M$=$0$)}
  \label{tbl:ablution}
  \centering
  %\vspace{-5pt}
  \begin{threeparttable}
    \begin{footnotesize}
      \begin{tabular}{
        @{\hspace{0pt}}c@{\hspace{8pt}}
        @{\hspace{8pt}}c@{\hspace{8pt}}
        %  
        @{\hspace{8pt}}r@{\hspace{8pt}}
        %
        @{\hspace{8pt}}r@{\hspace{8pt}}
        %
        @{\hspace{8pt}}r@{\hspace{0pt}}
        }
        \toprule
        %\multirow{2}{*}{$\LL$} & \multirow{2}{*}{$\T$}
        %&\multicolumn{2}{c}{CDs} && \multicolumn{2}{c}{Comics}\\
        %\cline{3-4}\cline{6-7}
        %&& \scriptsize{Recall@5} & \scriptsize{Recall@10} && \scriptsize{Recall@5} & \scriptsize{Recall@10}\\
        %\midrule
        %\multirow{5}{*}{2}
       $\LL$ & $\T$ & CDs && Comics\\
       \midrule
       \multirow{4}{*}{2}
       %& 1 & 0.0294 
       %& 1 & 0.0483 %&& 0.0997 
       %&& 0.1491\\
       %& 2 & \underline{0.0299} 
       & 2 & \underline{0.0487} %&& 0.1085 
       && 0.1588\\
       %& 3 & 0.0288 
       & 3 & 0.0482 %&& 0.1100 
       && 0.1613\\
       %& 4 & 0.0297 
       & 4 & 0.0472 %&& \underline{0.1104} 
       && \underline{0.1620}\\
       %& 5 & 0.0280 
       & 5 & 0.0470 %&& 0.1082 
       && 0.1605\\
         \midrule
        \multirow{5}{*}{3}
        %& 1 & 0.0300 
        & 1 & 0.0484 %&& 0.0993 
        && 0.1486 \\
        %& 2 & \underline{\textbf{0.0302}} 
        & 2 & \underline{\textbf{0.0492}} %&& 0.1075 
        && 0.1585 \\
        %& 3 & {0.0301} 
        & 3 & 0.0481 %&& 0.1101 
        && 0.1607 \\
        %& 4 & 0.0299 
        & 4 & 0.0475 %&& \underline{\textbf{0.1107}} 
        && \underline{\textbf{0.1624}}\\
        %& 5 & 0.0288 
        & 5 & 0.0477 %&& 0.1103 
        && {0.1623}\\
       \midrule
        \multirow{4}{*}{4}
        %& 1 & 0.0298 
        %& 1 & 0.0483 %&& 0.0991 
        %&& 0.1481 \\
        %& 2 & \underline{0.0299} 
        & 2 & \underline{0.0491} %&& 0.1071 
        && 0.1584 \\
        %& 3 & 0.0296 
        & 3 & 0.0481 %&& 0.1094 
        && 0.1608 \\
        %& 4 & 0.0288 
        & 4 & 0.0463 %&& \underline{0.1104} 
        && \underline{0.1618}\\
        %& 5 & 0.0278 
        & 5 & 0.0461 %&& 0.1088 
        && 0.1600\\
%        \midrule
%        \multirow{5}{*}{5}
%        & 1 & 0.0286 & 0.0462 && 0.0982 & 0.1473 \\
%        & 2 & 0.0291 & 0.0473 && 0.1067 & 0.1568 \\
%        & 3 & 0.0293 & 0.0481 && 0.1081 & 0.1593 \\
%        & 4 & 0.0284 & 0.0467 && 0.1091 & 0.1603\\
%        & 5 & 0.0280 & 0.0447 && 0.1081 & 0.1597\\
%        \midrule
%        \multirow{5}{*}{6}
%        & 1 & 0.0279 & 0.0459 && 0.0954 & 0.1445\\
%        & 2 & 0.0277 & 0.0454 && 0.1036 & 0.1543\\
%        & 3 & 0.0285 & 0.0470 && 0.1071 & 0.1581\\
%        & 4 & 0.0284 & 0.0463 && 0.1068 & 0.1580\\
%        & 5 & 0.0276 & 0.0451 && 0.1060 & 0.1566\\
        \bottomrule
      \end{tabular}
   \end{footnotesize}
   %   \begin{tablenotes}[normal,flushleft]
   %   \begin{footnotesize}
   %   \item
   %       The best performance for each $\LL$ is \underline{underlined}.
   %       The best performance across all $\LL$ values is \textbf{bold}.
   %       \par
   %   \end{footnotesize}
   %   \end{tablenotes}
  \end{threeparttable}
\end{minipage}
%
%\quad
%~
%%
%\begin{minipage}[!t]{0.33\linewidth}
%
%  \centering
%  \input{./plots/data_distribution/data_distribution.tex}
%  \vspace{-8pt}
%  \captionof{figure}{Item Frequency Distribution}
%  \label{fig:total_distribution}
%  \vspace{-8pt}
%
%
%  \captionof{table}{\mbox{\methodMean Parameter Study  (\CUS, $\M$=$2$, $\T$=$3$)}}
%  \label{tbl:parameterT}
%  \centering
%  \vspace{1pt}
%  \begin{threeparttable}
%
%     \begin{footnotesize} 
%        \begin{tabular}{
%        @{\hspace{1pt}}c@{\hspace{1pt}}
%        %
%        @{\hspace{1pt}}c@{\hspace{1pt}}
%        @{\hspace{1pt}}r@{\hspace{1pt}}
%        %
%        @{\hspace{0pt}}r@{\hspace{0pt}}
%        %
%        @{\hspace{1pt}}r@{\hspace{1pt}}
%        @{\hspace{1pt}}r@{\hspace{1pt}}
%        }
%        \toprule
%        \multirow{2}{*}{$\LL$}
%        &\multicolumn{2}{c}{CDs} && \multicolumn{2}{c}{Comics}\\
%        \cline{2-3}\cline{5-6}
%        & \scriptsize{Recall@5} & \scriptsize{Recall@10} && \scriptsize{Recall@5} & \scriptsize{Recall@10}\\
%        \midrule
%         3 & 0.0358 & 0.0556 && 0.2384 & 0.3022\\
%         4 & \textbf{0.0369} & \textbf{0.0583} && 0.2402 & 0.3043\\
%         5 & 0.0366 & 0.0567 && \textbf{0.2414} & \textbf{0.3065}\\
%         6 & 0.0360 & 0.0572 && 0.2392 & 0.3063\\
%        \bottomrule
%      \end{tabular}
%   \end{footnotesize}
%      %\begin{tablenotes}[normal,flushleft]
%      %\begin{scriptsize}
%      %\item
%      %    The best performance for each $|T|$ is \underline{underlined}.
%      %    The best performance across all $|T|$ values is \textbf{bold}.
%      %    \par
%      %\end{scriptsize}
%      %\end{tablenotes}
%  \end{threeparttable}
%%
%\vspace{8pt}
%%
%%
%  \caption{\mbox{\methodMean Parameter Study (\LOS, $\M$=$2$, $\T$=$3$)}}
%  \label{tbl:parameterO}
%  \centering
%  \vspace{1pt}
%  \begin{threeparttable}
%   \begin{footnotesize}
%      \begin{tabular}{
%        @{\hspace{1pt}}c@{\hspace{1pt}}
%        %
%        @{\hspace{1pt}}c@{\hspace{1pt}}
%        @{\hspace{1pt}}r@{\hspace{1pt}}
%        %
%        @{\hspace{0pt}}r@{\hspace{0pt}}
%        %
%        @{\hspace{1pt}}r@{\hspace{1pt}}
%        @{\hspace{1pt}}r@{\hspace{1pt}}
%        }
%        \toprule
%        \multirow{2}{*}{$\LL$}
%        &\multicolumn{2}{c}{CDs} && \multicolumn{2}{c}{Comics}\\
%        \cline{2-3}\cline{5-6}
%        & \scriptsize{Recall@5} & \scriptsize{Recall@10} && \scriptsize{Recall@5} & \scriptsize{Recall@10}\\
%        \midrule
%%         3 & 0.0345 & 0.0541 && 0.1791 & 0.2289\\
%         4 & 0.0343 & 0.0544 && 0.1818 & 0.2317\\
%         5 & \textbf{0.0357} & \textbf{0.0565} && \textbf{0.1823} & \textbf{0.2331}\\
%         6 & 0.0355 & 0.0550 && 0.1821 & 0.2314\\
%        \bottomrule
%      \end{tabular}
%   \end{footnotesize}
%%      \begin{tablenotes}[normal,flushleft]
%%      \begin{scriptsize}
%%      \item
%%          The best performance for each $|L|$ is \underline{underlined}.
%%          The best performance across all $|L|$ values is \textbf{bold}.
%%          \par
%%      \end{scriptsize}
%%      \end{tablenotes}
%  \end{threeparttable}
%\end{minipage}
%  \vspace{-15pt}
\end{table}




==> tables/performance.tex <==
\begin{table}[!t]
\footnotesize
  \caption{Performance in \CUT ($|L|=5$, $|T|=3$, $|M|=2$)}
  \centering
  \label{tbl:performance}
  \vspace{-3pt}
  \begin{threeparttable}
      \begin{tabular}{
	@{\hspace{0pt}}l@{\hspace{3pt}}
	@{\hspace{3pt}}l@{\hspace{3pt}}          
	@{\hspace{3pt}}r@{\hspace{3pt}}
	@{\hspace{3pt}}r@{\hspace{3pt}}
	@{\hspace{3pt}}r@{\hspace{3pt}}
	@{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
    @{\hspace{3pt}}r@{\hspace{0pt}}
	}
        \toprule
         & Dataset & \Caser & \SASRec & \HGN & \methodMax & \methodMean & improv\\
        \midrule
 %       \multirow{6}{*}{R@10}
	 \multirow{6}{*}{\rotatebox[origin=c]{90}{{\centering Recall@10}}}
        & CDs & 0.0274 & 0.0376 & \underline{0.0445} & 0.0430 & \textbf{0.0508} & 14.16\%\\
        & Books & 0.0267 & 0.0365 & 0.0426 & \underline{0.0441} & \textbf{0.0477} & 11.97\%\\
        & Children & 0.1112 & 0.1204 & 0.1254 & \underline{0.1332} & \textbf{0.1350} & 7.66\%\\
        & Comics & 0.1476 & 0.1599 & 0.1733 & \underline{0.1789} & \textbf{0.1814} & 4.67\%\\
        & ML-20M & 0.1201 & 0.1073 & \underline{0.1264} & 0.1220 & \textbf{0.1284} & 1.58\%\\
        & ML-1M & \textbf{0.1291} & 0.1236 & 0.1233 & 0.1210 & \underline{0.1258} & -2.56\%\\
        \midrule
%        \multirow{6}{*}{N@10}
 \multirow{6}{*}{\rotatebox[origin=c]{90}{{\centering NDCG@10}}}
        & CDs & 0.0169 & 0.0202 & \underline{0.0233} & 0.0217 & \textbf{0.0259} & 11.16\%\\
        & Books & 0.0216 & 0.0260 & \underline{0.0316} & 0.0305 & \textbf{0.0324} & 2.53\%\\
        & Children & 0.1075 & 0.1130 & 0.1126 & \underline{0.1173} & \textbf{0.1195} & 6.13\%\\
        & Comics & 0.1777 & 0.1874 & 0.1910 & \underline{0.1938} & \textbf{0.1959} & 2.57\%\\
        & ML-20M & \textbf{0.1234} & 0.1072 & 0.1184 & 0.1149 & \underline{0.1213} & -1.70\%\\
        & ML-1M & \textbf{0.1636} & \underline{0.1579} & 0.1521 & 0.1477 & 0.1537 & -6.05\%\\
        \bottomrule
      \end{tabular}
            \begin{tablenotes}[normal,flushleft]
      \begin{scriptsize}
      \item
          The best performance in each dateset is \textbf{bold}.
          The second best performance in each dataset is \underline{underlined}. 
          The column ``Improv'' presents the improvement of best performance of 
          \method-based methods over the best performance of non-\method methods in each row.
          \par
      \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
\end{table}


==> tables/performance_combine.tex <==
\begin{table}[!h]
\footnotesize
  \caption{\mbox{Performance Comparison in \CUT ($\M$=$2$)}} %\xia{other parameters}) }}
  \centering
  \label{tbl:performance}
  %\vspace{-5pt}
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{0pt}}l@{\hspace{10pt}}
        @{\hspace{10pt}}l@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
    @{\hspace{10pt}}r@{\hspace{0pt}}
        }
        \toprule
         & Dataset & \Caser & \SASRec & \HGN & \methodMax & \methodMean & improv\\
        \midrule
 %       \multirow{6}{*}{R@10}
         \multirow{6}{*}{\rotatebox[origin=c]{90}{{\centering Recall@10}}}
        & CDs & 0.0291 & 0.0376 & \underline{0.0445} & 0.0430 & \textbf{0.0508} & 14.16\%\\
        & Books & 0.0295 & 0.0365 & 0.0426 & \underline{0.0441} & \textbf{0.0477} & 11.97\%\\
        & Children & 0.1161 & 0.1204 & 0.1254 & \underline{0.1332} & \textbf{0.1350} & 7.66\%\\
        & Comics & 0.1580 & 0.1599 & 0.1733 & \underline{0.1789} & \textbf{0.1823} & 4.67\%\\
        & ML-20M & 0.1235 & 0.1073 & \underline{0.1264} & 0.1220 & \textbf{0.1284} & 1.58\%\\
        & ML-1M & \textbf{0.1317} & 0.1236 & 0.1233 & 0.1210 & \underline{0.1258} & -4.48\%\\
        \midrule
%        \multirow{6}{*}{N@10}
 \multirow{6}{*}{\rotatebox[origin=c]{90}{{\centering NDCG@10}}}
        & CDs & 0.0176 & 0.0202 & \underline{0.0233} & 0.0217 & \textbf{0.0259} & 11.16\%\\
        & Books & 0.0235 & 0.0260 & \underline{0.0316} & 0.0305 & \textbf{0.0324} & 2.53\%\\
        & Children & 0.1118 & 0.1130 & 0.1126 & \underline{0.1173} & \textbf{0.1195} & 6.13\%\\
        & Comics & 0.1886 & 0.1874 & 0.1910 & \underline{0.1938} & \textbf{0.1959} & 2.57\%\\
        & ML-20M & \textbf{0.1266} & 0.1072 & 0.1184 & 0.1149 & \underline{0.1213} & -4.19\%\\
        & ML-1M & \textbf{0.1655} & \underline{0.1579} & 0.1521 & 0.1477 & 0.1537 & -7.13\%\\
        \bottomrule
      \end{tabular}
%      \begin{tablenotes}[normal,flushleft]
%      \begin{scriptsize}
%      \item
%          The best performance in each dateset is \textbf{bold}.
%          The second best performance in each dataset is \underline{underlined}.
%          The column ``improv'' presents the improvement of best performance of
%          \method-based methods over the best performance of non-\method methods in each row.
%          \par
%      \end{scriptsize}
%      \end{tablenotes}
  \end{threeparttable}





%\vspace{5pt}






\footnotesize
  \caption{\mbox{Performance Comparison in \CUS ($\M$=$2$, $\T$=$3$)}}
  \centering
  \label{tbl:near}
  %\vspace{-5pt}
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{0pt}}l@{\hspace{10pt}}
        @{\hspace{10pt}}l@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
    @{\hspace{10pt}}r@{\hspace{0pt}}
        }
        \toprule
        & Dataset & \Caser & \SASRec & \HGN & \methodMax & \methodMean & improv\\
        \midrule
        %\multirow{6}{*}{R@10}
        \multirow{6}{*}{\rotatebox[origin=c]{90}{{\centering Recall@10}}}
        & CDs & 0.0340 & 0.0402 & \underline{0.0508} & 0.0488  & \textbf{0.0583} & 14.76\%\\
        & Books & 0.0384 & 0.0473 & 0.0573 & \underline{0.0596} & \textbf{0.0625} & 9.08\%\\
        & Children & 0.1622 & 0.1773 & \underline{0.1980} & 0.1961 & \textbf{0.2008} & 1.41\%\\
        & Comics & 0.2012 & 0.2801 & \underline{0.3055} & 0.3003 & \textbf{0.3065} & 0.33\%\\
        & ML-20M & \textbf{0.1779} & 0.1368 & 0.1655 & 0.1605  & \underline{0.1690} & -5.00\%\\
        & ML-1M & 0.1830 & 0.1963 & \underline{0.2045} & 0.1950 & \textbf{0.2083} & 1.86\%\\
        \midrule
        %\multirow{6}{*}{N@10}
        \multirow{6}{*}{\rotatebox[origin=c]{90}{{\centering NDCG@10}}}
        & CDs & 0.0133 & 0.0149 & \underline{0.0211} & 0.0198 & \textbf{0.0240} & 13.74\%\\
        & Books & 0.0163 & 0.0188 & 0.0241 & \underline{0.0249} & \textbf{0.0260} & 7.88\%\\
        & Children & 0.0703 & 0.0846 & \textbf{0.1054} & 0.1036 & \underline{0.1051} & -0.28\%\\
        & Comics & 0.1070 & 0.1621 & \textbf{0.2040} & 0.1942 &\underline{0.1982} & -2.84\%\\
        & ML-20M & \textbf{0.0713} & 0.0530 & 0.0674 & 0.0665 & \underline{0.0707} & -0.84\%\\
        & ML-1M & 0.0763 & 0.0801 & \underline{0.0852} & 0.0802 & \textbf{0.0883} & 3.64\%\\
        \bottomrule
      \end{tabular}
%      \begin{tablenotes}[normal,flushleft]
%      \begin{scriptsize}
%      \item
%          The best performance in each dateset is \textbf{bold}.
%          The second best performance in each dataset is \underline{underlined}.
%          The column ``improv'' presents the improvement of best performance of
%          \method-based methods over the best performance of non-\method methods in each row.
%          \par
%      \end{scriptsize}
%      \end{tablenotes}
  \end{threeparttable}



%\vspace{5pt}




\footnotesize
  \caption{\mbox{Performance Comparison in \LOS ($\M$=$2$, $\T$=$3$)}}
  \centering
  \label{tbl:performancelevel}
  %\vspace{-5pt}
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{0pt}}l@{\hspace{10pt}}
        @{\hspace{10pt}}l@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
    @{\hspace{10pt}}r@{\hspace{0pt}}
        }
        \toprule
        & Dataset & \Caser & \SASRec & \HGN & \methodMax & \methodMean & improv\\
        \midrule
        %\multirow{6}{*}{R@10}
        \multirow{6}{*}{\rotatebox[origin=c]{90}{{\centering Recall@10}}}
        & CDs & 0.0306 & 0.0412 & 0.0493 & \underline{0.0497} & \textbf{0.0565} & 14.60\%\\
        & Books & 0.0327 & 0.0506 & 0.0517 & \underline{0.0550} & \textbf{0.0576} & 11.41\%\\
        & Children & 0.1241 & 0.1349 & \underline{0.1473} & 0.1467 & \textbf{0.1503} & 2.04\%\\
        & Comics & 0.1984 & 0.2196 & \textbf{0.2366} & 0.2271 & \underline{0.2331} & -1.48\%\\
        & ML-20M & 0.1393 & 0.1259 & \underline{0.1461} & 0.1420  & \textbf{0.1489} & 1.92\%\\
        & ML-1M & \underline{0.1794} & 0.1635 & 0.1762 & 0.1736 & \textbf{0.1818} & 1.34\%\\
        \midrule
        %\multirow{6}{*}{N@10}
        \multirow{6}{*}{\rotatebox[origin=c]{90}{{\centering NDCG@10}}}
        & CDs & 0.0112 & 0.0156 & \underline{0.0205} & 0.0203 & \textbf{0.0239} & 16.59\%\\
        & Books & 0.0131 & 0.0211 & 0.0211 & \underline{0.0226} & \textbf{0.0236} & 11.85\%\\
        & Children & 0.0622 & 0.0646 & \underline{0.0753} & 0.0737 & \textbf{0.0763} & 6.13\%\\
        & Comics & 0.1219 & 0.1321 & \textbf{0.1564} & 0.1458 & \underline{0.1486} & -4.99\%\\
        & ML-20M & 0.0561 & 0.0484 & \underline{0.0601} & 0.0587 & \textbf{0.0624} & 3.83\%\\
        & ML-1M & \underline{0.0769} & 0.0670 & 0.0761 & 0.700 & \textbf{0.0780} & 1.43\%\\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}[normal,flushleft]
      \begin{scriptsize}
      \item
          In the above three tables, the best performance in each dateset is \textbf{bold}.
          The second best performance in each dataset is \underline{underlined}.
          The column ``improv'' presents the improvement of best performance of
          \method-based methods over the best performance of non-\method methods in each row.
          \par
      \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
  %\vspace{-10pt}
\end{table}





==> tables/performance_levelout.tex <==
\begin{table}[!h]
\footnotesize
  \caption{Performance Comparison on levelout setting}
  \centering
  \label{tbl:performancelevel}
  \vspace{-3pt}
  \begin{threeparttable}
      \begin{tabular}{
	@{\hspace{0pt}}l@{\hspace{3pt}}
	@{\hspace{3pt}}l@{\hspace{3pt}}          
	@{\hspace{3pt}}r@{\hspace{3pt}}
	@{\hspace{3pt}}r@{\hspace{3pt}}
	@{\hspace{3pt}}r@{\hspace{3pt}}
	@{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
    @{\hspace{3pt}}r@{\hspace{0pt}}
	}
        \toprule
        & Dataset & Caser & SASRec & HGN & MAX & MEAN & Improv\\
        \midrule
        %\multirow{6}{*}{R@10}
        \multirow{6}{*}{\rotatebox[origin=c]{90}{{\centering Recall@10}}}
        & CDs & 0.0306 & 0.0412 & 0.0493 & \underline{0.0497} & \textbf{0.0565} & 14.60\%\\
        & Books & 0.0327 & 0.0506 & 0.0517 & \underline{0.0550} & \textbf{0.0576} & 11.41\%\\
        & Children & 0.1241 & 0.1349 & \underline{0.1473} & 0.1467 & \textbf{0.1503} & 2.04\%\\
        & Comics & 0.1984 & 0.2196 & \textbf{0.2366} & 0.2271 & \underline{0.2331} & -1.48\%\\
        & ML-20M & 0.1393 & 0.1259 & \underline{0.1461} & 0.1420  & \textbf{0.1489} & 1.92\%\\
        & ML-1M & \underline{0.1794} & 0.1635 & 0.1762 & 0.1736 & \textbf{0.1818} & 1.34\%\\
        \midrule
        %\multirow{6}{*}{N@10}
        \multirow{6}{*}{\rotatebox[origin=c]{90}{{\centering NDCG@10}}}
        & CDs & 0.0112 & 0.0156 & \underline{0.0205} & 0.0203 & \textbf{0.0239} & 16.59\%\\
        & Books & 0.0131 & 0.0211 & 0.0211 & \underline{0.0226} & \textbf{0.0236} & 11.85\%\\
        & Children & 0.0622 & 0.0646 & \underline{0.0753} & 0.0737 & \textbf{0.0763} & 6.13\%\\
        & Comics & 0.1219 & 0.1321 & \textbf{0.1564} & 0.1458 & \underline{0.1486} & -4.99\%\\
        & ML-20M & 0.0561 & 0.0484 & \underline{0.0601} & 0.0587 & \textbf{0.0624} & 3.83\%\\
        & ML-1M & \underline{0.0769} & 0.0670 & 0.0761 & 0.700 & \textbf{0.0780} & 1.43\%\\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{small}
	\item
          The bset performance in each dateset is \textbf{bold}.
          The second best performance in each dataset is \underline{underlined}. 
          The column ``Improv'' presents the improvement of best performance of
          \method-based methods over the best performance of non-\method methods in each row.
          \par
	\end{small}
      \end{tablenotes}
  \end{threeparttable}
\end{table}


==> tables/performance_near.tex <==
\begin{table}[!t]
\footnotesize
  \caption{Performance Comparison in \CUS}
  \centering
  \label{tbl:near}
  \vspace{-3pt}
  \begin{threeparttable}
      \begin{tabular}{
	@{\hspace{0pt}}l@{\hspace{3pt}}
	@{\hspace{3pt}}l@{\hspace{3pt}}          
	@{\hspace{3pt}}r@{\hspace{3pt}}
	@{\hspace{3pt}}r@{\hspace{3pt}}
	@{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
    @{\hspace{3pt}}r@{\hspace{0pt}}
	}
        \toprule
        & Dataset & Caser & SASRec & HGN & MAX & MEAN & Improv\\
        \midrule
        %\multirow{6}{*}{R@10}
        \multirow{6}{*}{\rotatebox[origin=c]{90}{{\centering Recall@10}}}
        & CDs & 0.0340 & 0.0402 & \underline{0.0508} & 0.0488  & \textbf{0.0583} & 14.76\%\\
        & Books & 0.0384 & 0.0473 & 0.0573 & \underline{0.0596} & \textbf{0.0625} & 9.08\%\\
        & Children & 0.1622 & 0.1773 & \underline{0.1980} & 0.1961 & \textbf{0.2008} & 1.41\%\\
        & Comics & 0.2012 & 0.2801 & \underline{0.3055} & 0.3003 & \textbf{0.3065} & 0.33\%\\
        & ML-20M & \textbf{0.1779} & 0.1368 & 0.1655 & 0.1605  & \underline{0.1690} & -5.00\%\\
        & ML-1M & 0.1775 & 0.1963 & \underline{0.2045} & 0.1950 & \textbf{0.2083} & 1.86\%\\
        \midrule
        %\multirow{6}{*}{N@10}
        \multirow{6}{*}{\rotatebox[origin=c]{90}{{\centering NDCG@10}}}
        & CDs & 0.0133 & 0.0149 & \underline{0.0211} & 0.0198 & \textbf{0.0240} & 13.74\%\\
        & Books & 0.0163 & 0.0188 & 0.0241 & \underline{0.0249} & \textbf{0.0260} & 7.88\%\\
        & Children & 0.0703 & 0.0846 & \textbf{0.1054} & 0.1036 & \underline{0.1051} & 0.28\%\\
        & Comics & 0.1070 & 0.1621 & \textbf{0.2040} & 0.1942 &\underline{0.1982} & -2.84\%\\
        & ML-20M & \textbf{0.0713} & 0.0530 & 0.0674 & 0.0665 & \underline{0.0707} & 0.84\%\\
        & ML-1M & 0.0714 & 0.0801 & \underline{0.0852} & 0.0802 & \textbf{0.0883} & 3.64\%\\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{small}
	\item
          The bset performance in each dateset is \textbf{bold}.
          The second best performance in each dataset is \underline{underlined}. 
          The column ``Improv'' presents the improvement of best performance of
          \method-based methods over the best performance of non-\method methods in each row.
          \par
	\end{small}
      \end{tablenotes}
  \end{threeparttable}
\end{table}


==> tables/times_train.tex <==
\begin{table}[h!]
\footnotesize
  \caption{\mbox{{Training-Time Performance in {\CUT} (seconds)}}}
  \centering
  \label{tbl:timeTrain}
  %\vspace{-5pt}
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{8pt}}l@{\hspace{8pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
        @{\hspace{4pt}}r@{\hspace{8pt}}
        @{\hspace{12pt}}r@{\hspace{8pt}}
        @{\hspace{12pt}}r@{\hspace{4pt}}
        @{\hspace{4pt}}r@{\hspace{8pt}}
        }
        \toprule
         Dataset & \Caser & \SASRec & \HGN & \methodCorm & speedup\\
        \midrule
	CDs      & 7.4e-4 & 3.0e-3 & \textbf{1.4e-4} & \underline{1.8e-4} & 0.78\\
        Books    & 1.2e-3 & 2.9e-3 & \underline{3.0e-4} & \textbf{2.7e-4} & 1.11\\
        Children & 1.5e-3 & 8.7e-4 & \textbf{2.8e-4} & \underline{4.4e-4} & 0.64\\
        Comics   & 1.8e-3 & 1.8e-3 & \textbf{3.3e-4} & \underline{5.5e-4} & 0.60\\
        ML-20M   & 2.2e-3 & 2.4e-3 & \textbf{2.7e-4} & \underline{8.1e-4} & 0.33\\
        ML-1M    & 3.5e-3 & 1.5e-3 & \textbf{2.7e-4} & \underline{5.4e-4} & 0.50\\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}[normal,flushleft]
      \begin{scriptsize}
      \item
          In the above table, the best training-time performance in each dateset is \textbf{bold}.
          The second best training-time performance in each dataset is \underline{underlined}.
          The column ``speedup'' presents the speedup of the \textbf{bold} best performance
          over the \underline{underlined} second best performance in each dataset.
          \par
      \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
  \vspace{-5pt}
\end{table}


==> tem.tex <==
We implement \method in python with pytorch 1.2.0 (https://pytorch,org).
  We used Adam optimizer with learning rate 1e-3 and
  regularization factor 1e-3 on all the datasets.
  The dimension of embeddings $d$,
  the number of items in high-order/low-order associations $\LL$/$\M$,
  the number of items to be recommended used for training $\T$,
  and the order of item synergies that are specific for each dataset are reported in
  Table~\ref{tbl:para:ham}
  %
  For \HGN, we used the implementation
  provided by the authors in github~\footnote{\url{https://github.com/allenjack/HGN}},
  we used the default Adam optimizer with learning rate 1e-3 and
  regularization factor 1e-3 on all the datasets.
  The dimension of embeddings $d$,
  the length of the subsequences $L$
  and the number of items used as targets in training $T$ of each dataset
  are reported in Table~\ref{tbl:para:hgn}.
  %
  For \SASRec, we used the implementation provided by the authors in
  github~\footnote{\url{https://github.com/kang205/SASRec}}
  as well.
  We used the default Adam optimizer with learning rate 1e-3 and
  the exponential decay rate for the second-moment estimates beta2 0.98.
  The dimension of embeddings $d$,
  the maximum sequence length $n$
  and the number of heads of the multi-head attention $h$ of each dataset
  are reported in Table~\ref{tbl:para:sasrec}.
  %
  For \Caser, we also used the pytorch implementation suggested by the authors in
  github~\footnote{\url{https://github.com/graytowne/caser_pytorch}}.
  We used the default Adam optimizer with learning rate 1e-3
  and regularization factor 1e-6.
  The dimension of embeddings $d$,
  the length of the subsequences $L$,
  the number of items used as targets in training $T$,
  the number of vertical filters in CNNs $nv$
  and the number of horizontal filters in CNNs $nh$ of each dataset
  are reported in Table~\ref{tbl:para:caser}

